Noise Map Guidance: Inversion with Spatial Context for Real Image Editing

Text-guided diffusion models have become a popular tool in image synthesis, known for producing high-quality and diverse images. However, their application to editing real images often encounters hurdles primarily due to the text condition deteriorating the reconstruction quality and subsequently affecting editing fidelity. Null-text Inversion (NTI) has made strides in this area, but it fails to capture spatial context and requires computationally intensive per-timestep optimization. Addressing these challenges, we present Noise Map Guidance (NMG), an inversion method rich in a spatial context, tailored for real-image editing. Significantly, NMG achieves this without necessitating optimization, yet preserves the editing quality. Our empirical investigations highlight NMG's adaptability across various editing techniques and its robustness to variants of DDIM inversions.

==> 7_rebuttal_comments.tex <==
\begin{center}
    \Large
    \textbf{Rebuttal Response} \\
\end{center}


\textbf{Overall Response}


Thank you for the reviewers' valuable insights and constructive feedback on our manuscript. We have thoughtfully considered suggestions and have made several significant improvements to enhance the clarity and depth of our work. Newly added sections are highlighted in blue for ease of reference.

\textbf{Improvement of Figure 2 (reviwer 9KmB)}: We have revised Figure 2 to provide a more precise and comprehensive visual representation. This improved figure now better demonstrates the capabilities and advantages of our NMG, particularly in comparison to NTI. The enhancements in this figure aim to address the previously noted ambiguities and provide a more intuitive understanding of our method’s functionality.

\textbf{Additional Results of Section A.4 and Figure 8 in the Appendix (reviwer 9KmB)}: 
In response to the need for additional experimental results, we have included Figure 8 and an accompanying description in Section A.4. This section provides a thorough comparative analysis with ProxNPI, an in-depth analysis of combining NMG with NTI, and additional reconstruction results and user study findings.

\textbf{Inclusion of Section B in the Appendix}: Section B has been included to discuss our work's limitations and potential future directions. Here, we address challenges in editing tasks that require significant modifications to spatial structures. This section aims to provide a transparent and honest assessment of our method's capabilities and outlines areas for future research and development.

These updates have been made to address the key concerns and suggestions raised by the reviewers. We believe that these improvements significantly augment the quality of our manuscript, providing more precise insights into our method's strengths, limitations, and potential for future advancement.


\newpage
\textbf{Reviewer1(yyX5)}

\textbf{[W1]} The visualization results depict many recurring stylization outcomes, such as the "oil painting style" and "Van Gogh style". It would be beneficial for the paper to exhibit a broader variety of more challenging editing instances.

>> We have newly appended additional stylization results in Figure 8(a) and a description to Section A.4 in the Appendix of the revised paper. In this figure, we present additional results that showcase NMG's capabilities in handling a wide range of artistic styles, extending well beyond the initially noted painting stylizations. Specifically, the figure includes examples of editing outcomes in styles like anime and mosaic. This diversity in style adaptation illustrates the flexibility and robustness of NMG in accommodating various artistic expressions and editing challenges.

\textbf{[W2]} The user study could benefit from providing more accurate directives in its questions; if it pertains to local editing, for instance, the question should contemplate including "evaluate original preservation in unedited areas.”

>> We agree that a precise evaluation framework is crucial for assessing the performance of our method. To this end, we have conducted an additional user study and have detailed the methodology and results in Section A.4 and Table 3 in the Appendix of the revised paper. This study is designed with a particular focus on evaluating the preservation of integrity in unedited areas during local editing tasks and the retention of overall structure in global editing scenarios. As evidenced in Table 3, the outcomes affirm that NMG successfully maintains unedited regions during local editing tasks and preserves the overarching structure in global edits, underlining its effectiveness in diverse editing contexts.

\textbf{[Q1]} How about the editing performance of adding or deleting elements in the images?

>> We have added additional results in Figure 9(c) in the revised paper. NMG can eliminate objects from an image, such as removing a person. 

However, it is essential to note that while NMG can successfully execute such deletions, it is currently limited in its specificity when selecting individual targets for removal. Similarly, NMG faces challenges in adhering to detailed locational instructions when adding new objects to an image. Although NMG provides reliable editing for general tasks, its reliance on text for image editing introduces difficulties in executing detailed spatial changes.
We have added this discussion in Section B of the revised paper as a limitation discussion.


\textbf{[Q2]} While both global and local editing in the ProxNPI paper seem promising, the editing capability in this paper doesn't appear as effective. For instance, in Figure 3, the second row shows an edited result with a clear boundary between two types of backgrounds. In the third row, under "Van Gogh," the overall style seems to have undergone minimal change. Can you provide an explanation for these observations?

>> We have conducted an additional comparison with ProxNPI, illustrated in Figure 8(d) and thoroughly discussed in Section A.4 in the revised paper. This comparison reveals that NMG achieves results on par with those showcased in the ProxNPI study. However, it is essential to note that ProxNPI does not extensively explore various editing scenarios, such as contextual alterations or stylization. In contrast, NMG has demonstrated its proficiency across a wide range of editing scenarios. 

Additionally, as elaborated in Section 4.1, ProxNPI faces limitations due to its dependence on inversion guidance. NMG, free from such constraints, exhibits greater versatility and effectiveness in various image editing tasks, underscoring its broader applicability and utility in the field of image editing.

Note that ProxNPI was an unpublished arxiv work at the time of our submission, and our work was independently developed in parallel(i.e., concurrent work). While ProxNPI may be a noteworthy project, we may believe it'd be unfair to us to be discounted by ProxNPI with a single perspective. Our research offers unique insights and contributions that stand on their own merit and we respectfully ask an unbiased evaluation by the reviewer, considering this matter.



\newpage
\textbf{Reviewer2(9KmB)}

\textbf{[W1]} Figure 2 seems confusing to me. Since this paper repeatedly mentioned that NMG address the challenges in Null-text Inversion, I think it would be nice to compare NMG to Null-text Inversion in this Figure, and demonstrate how NMG outperforms Null-text Inversion. In addition, it would be nice to add the corresponding text descriptions in the Figure. E.g., it's unclear whether the caption indicate to change the blue fire hydrant to a red one or it's just some deviations during the reconstruction.

>> Thank you for insightful feedback on Figure 2. We acknowledge the necessity of clearly demonstrating how our NMG approach effectively addresses the challenges associated with NTI. In response to suggestions, we have revised Figure 2 for enhanced clarity. In the updated Figure 2(a), we illustrate the common divergence issues encountered in 
% naive reconstruction processes.
naive reconstruction with an unaligned reverse process.
This part of the figure highlights how such reconstructions often fail due to a deviation from the original inversion path, necessitating an alignment to achieve reliable reconstruction, which motivates our work.  Figure 2(b) then delves into the alignment process via NTI, which optimizes the null-text embedding to reduce the disparity between the inversion and reconstruction paths. However, NTI's reliance on a single vector of
% single-dimensional 
the null-text embedding for alignment 
% can
lead to challenges in preserving the spatial context of the input image due to having no spatial dimension of the null-text embedding.
In contrast, as shown in Figure 2(c), our NMG offers a novel approach to alignment. Our method
% refines
corrects the reconstruction path by conditioning it on the discrepancies between the inversion and reconstruction paths. NMG utilizes a noise map for this process, which inherently contains a richer spatial context than that of the null text embedding. This direct use of the noise map in NMG allows for more effective preservation of the spatial context during the editing process.

\textbf{[W2]} Limitations and future work should be discussed. For example, whether NMG can address the relationship change task like SGC-Net [1]? Whether NMG can achieve various non-rigid image editing tasks like Imagic [2]? It seems that NMG can achieve some non-rigid editing tasks such as viewpoint alternation or face expression modification. However, spatial information between the output and input>t seems consistent in the majority parts, from my view. Thus, it would be great to see experiments exploring whether NMG can perform other operations (with more obvious spatial information change) such as "from a tiger" to "a jumping/running tiger".

>> Thank you for the question regarding the capabilities of NMG. We acknowledge the importance of discussing our work's limitations and potential future directions.

[W2-1]
We have appended the limitation section in Section B, Appendix of the revised paper. As detailed in Section B, our current methodology is primarily designed to enhance inversion-based editing methods, focusing on improving spatial context during the editing process. However, NMG faces challenges integrating with methods like SGC-Net, which operates on a text-guided diffusion model for relationship change tasks; thus, not compatible with our current method. This is due to SGC-Net's deviation from the inversion-based editing paradigm, and it is non-trivial to design the integration.
% As a result, applying NMG for tasks involving relationship changes encounters significant hurdles. 
% For instance, as depicted in Figure 9(a), when attempting relationship change tasks using MasaCtrl, the results were ineffective as MasaCtrl is not inherently designed for such tasks.
As an alternative, we attempted relationship change tasks using MasaCtrl in Figure 9(a) in the Appendix of the revised paper. However, Figure 9(a) depicts the ineffectiveness of this approach, as MasaCtrl is not inherently designed for relationship change tasks. Consequently, NMG fails to conduct relationship change tasks.

[W2-2]
% Regarding the capabilities of NMG in handling various non-rigid image editing tasks, Figure 8(b) provides insights into this aspect.
We have conducted additional edited results of the non-rigid image editing task in Figure 8(b) in the revised paper. Figure 8(b) shows that NMG effectively conducts edits with pronounced spatial information changes, like standing to sitting and running to standing.

\newpage
\textbf{Reviewer3(pVhT)}

\textbf{[W1]} NMG impose a very strong spatial constraint during editing, as in the figure most showcase have almost the same geometry structure as the original picture, for case the modify geometry e.g. the cat in figure 4, the result shows an apparent artifacts in the modified region. There needs a further investigation on how will NMG perform when facing editing that requires modification on the spatial structure, for example removing a target (like "two man ..." ->"one man...") or change to a totally different object ("...car" to "... bike " ).
Moreover, there lack of discussion about possible failure cases of NMG, the authors should add such discussion about in what circumstance NMG would fail and the reason why it fails to help the community better understand the proposed method.

>> We have newly appended additional editing results that modify the spatial structure of the object in Figure 9(b) and (c) in the revised paper. Figure 9(b) underscores NMG's challenges in tasks that demand significant object structural changes. This is partly due to the inherent limitations of the inversion-based methods upon which NMG's editing capabilities are built. For instance, in Prompt-to-Prompt editing, the method involves swapping cross-attention maps between source and target texts. This approach inherently limits the scope of structural changes to those permissible within the constraints of the original object’s geometry. Additionally, as shown in Figure 9(c), we encounter limitations when removing specific targets. While NMG can eliminate an object from an image, the method often lacks the precision needed for detailed locational choices, making it challenging to select and remove specific targets. These examples highlight areas where NMG, in its current form, struggles to perform edits that require detailed spatial adjustments or significant geometric transformations. We have added this discussion in Section B of the revised paper as a limitation discussion.



\textbf{[Q1]} Why there are no quantitive and qualitative comparison with previous works about reconstruction? I think there should be a comparison with other methods in this aspect, or the author should explain why it is omitted.

>> Thank you for the question regarding the absence of comparisons with previous works, specifically in the context of reconstruction.
% While we offer a quantitative comparison of reconstruction capabilities in Table 3, 
We newly appended an additional quantitative comparison of reconstruction in Table 3 in the Appendix of the revised paper. NMG shows comparable performance with the comparison method in reconstruction.
It's important to emphasize that NMG focuses primarily on image editing rather than reconstruction. This distinction is pivotal as we aim to advance the field of image editing, where the quality of editing does not necessarily correlate directly with the quality of reconstruction. For instance, as shown in the sixth row of Figure 11, while ProxNPI exhibits commendable reconstruction ability, its editing capabilities are somewhat limited, highlighting the difference between reconstruction proficiency and editing versatility. We have added this discussion in Section A.4 in the Appendix of the revised paper.



\textbf{[Q2]} How NTI + NMG performs when dealing with actual editing task? it would be helpful to show the proposed method can combine with previous method to achieve a better result.

>> We have conducted additional experiments to explore how the synergy between NTI and NMG translates to actual image editing tasks. As shown in Figure 8(c), we observed that while NMG alone is a reliable tool for editing, it sometimes falls short in capturing specific spatial details. However, when we integrate additional information from NTI with NMG, this shortfall is effectively compensated for, enhancing the spatial context preservation in the edited images. This integration of NTI and NMG has shown promising results in our experiments, indicating a significant improvement in the editing capabilities of NMG. Thanks for the suggestion, which indeed improves our work further.

==> tables/edit.tex <==
\begin{table}
    \centering
    \begin{tabular}{l|cc|cc|cc|cc}
    \hline
    \multirow{2}{*}{Models} & \multicolumn{2}{c|}{P2P (Local)} & \multicolumn{2}{c|}{P2P (Global)} & \multicolumn{2}{c|}{MasaCtrl} & \multicolumn{2}{c}{Pix2Pix-zero} \\
    & CLIP$\uparrow$ & TIFA$\uparrow$ & CLIP$\uparrow$ & TIFA$\uparrow$ & CLIP$\uparrow$ & TIFA$\uparrow$ \\
    \hline
    DDIM & 0.2977 & 0.8436 & 0.3066 & 0.8349 & 0.2825 & 0.8253 \\
    NTI & 0.2983 & \textbf{0.9125} & 0.3202 & 0.8302 & 0.2903 & 0.8277 \\
    NPI & 0.2982 & 0.9076 & 0.3157 & 0.8117 & 0.2921 & 0.8188 \\
    ProxNPI & 0.2951 & 0.8947 & 0.3006 & 0.8463 & 0.2922 & 0.8188 \\
    \textbf{NMG(Ours)} & \textbf{0.3007} & 0.8955 & \textbf{0.3221} & \textbf{0.8991} & \textbf{0.2955} & \textbf{0.8548} \\
    \hline
    \end{tabular}
    \caption{Quantitative comparison on image editing.}
    \label{table:edit}
\end{table}

% \begin{table}
%     \centering
%     \begin{tabular}{l|ccccc|ccccc}
%     \hline
%     \multirow{2}{*}{Task} & \multicolumn{5}{c|}{P2P(Photorealistic)} & \multicolumn{5}{c}{P2P(Non-Photorealistic)} \\
%     & LPIPS$\downarrow$ & CLIP-I$\uparrow$ & SD$\downarrow$ & CLIP$\uparrow$ & TIFA$\uparrow$ & LPIPS$\downarrow$ & CLIP-I$\uparrow$ & SD$\downarrow$ & CLIP$\uparrow$ & TIFA$\uparrow$ \\
%     \hline
%     DDIM & 0.4874 & 0.7904 & 0.0617 & 0.2965 & 0.8449 & 0.5870 & 0.7255 & 0.0613 & 0.3089 & 0.8312 \\
%     NTI & 0.2127 & 0.8912 & 0.0106 & 0.2941 & \textbf{0.9031} & 0.4410 & 0.7415 & 0.0292 & 0.3179 & 0.8701 \\
%     NPI & 0.2571 & 0.8650 & 0.0187 & 0.2956 & 0.8988 & 0.4476 & 0.7278 & 0.0320 & 0.3114 & 0.8275 \\
%     ProxNPI & \textbf{0.1825} & \textbf{0.8974} & \textbf{0.0087} & 0.2923 & 0.8738 & \textbf{0.2810} & \textbf{0.8268} & \textbf{0.0154} & 0.2892 & 0.8470 \\
%     \textbf{NMG(Ours)} & 0.2635 & 0.8832 & 0.0123 & \textbf{0.3000} & 0.8910 & 0.5008 & 0.7397 & 0.0295 & \textbf{0.3223} & \textbf{0.8957} \\
%     \hline
    % \multirow{2}{*}{Task} & \multicolumn{5}{c|}{MasaCtrl} & \multicolumn{5}{c}{Pix2Pix-zero} \\
    % & LPIPS$\downarrow$ & CLIP-I$\uparrow$ & SD$\downarrow$ & CLIP$\uparrow$  & TIFA$\uparrow$ & LPIPS$\downarrow$ & CLIP-I$\uparrow$ & SD$\downarrow$ & CLIP$\uparrow$  & TIFA$\uparrow$ \\
    % \hline
    % DDIM & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    % NTI & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    % NPI & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    % ProxNPI & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    % \textbf{NMG(Ours)} & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 & 00.00 \\
    % \hline 
%     \end{tabular}
%     \caption{Quantitative comparison. Editing}
%     \label{table:quant_comp_recon}
% \end{table}
